On chain rule and renormalization

We discuss the relationship between the chain rule for the divergence operator and the renormalization property for weak solutions of the continuity equation. We construct an example of bounded divergence-free vector field on the plane, which demonstrates that in general the first property is not sufficient for the second one.

==> include/pic2b.tex <==
%\documentclass[border={5pt 5pt 5pt 5pt}]{standalone}
%\usepackage{tikz}
%
%\begin{document}
\begin{tikzpicture}
\node[font=\large] at (-4,10) {(b)};

% E
\draw[dashed, fill=black!10] (-3,0) -- (-3,3) -- (3,9) -- (3,0) -- cycle;

% Level sets
\foreach \y in {0, 0.75, ..., 3} {
    \draw[thick, color=black!30] (-3,\y) -- (3,\y*3);
}

% Axis
\draw[->] (-4,0) -- (4,0);
\node[font=\large,anchor = west] at (4,0) {$x_1$};
\draw[->] (0,0) -- (0,10);
\node[font=\large,anchor = south] at (0,10) {$x_2$};

% Subscriptions
\draw[thin, black!20] (-1,0) -- (0.5,-1);
\node[font=\Large,anchor=west] at (0.5,-1) {$f_n=t$};

\draw[thin, black!20] (-2,4) -- (-3.5,4.5);
\node[font=\Large,anchor=south] at (-3.5,4.5) {$f_n = t + \frac{1}{8} s_n$};

\node[font=\Large,anchor=north] at (3,0) {$a_n$};
\node[font=\Large,anchor=north] at (-3,0) {$-a_n$};

\draw[dotted] (0,3) -- (-3,3);
\node[font=\Large,anchor=west] at (0,3) {$b_n$};

\node[font=\Large,anchor=east] at (0,6) {$\frac{1}{8}d_n$};

\draw[dotted] (3,9) -- (0,9);
\node[font=\Large,anchor=east] at (0,9) {$\frac{1}{4}d_n - b_n$};

\end{tikzpicture}
%\end{document}

==> include/pic3.tex <==
%\documentclass[border={5pt 5pt 5pt 5pt}]{standalone}
%\usepackage{tikz}
%\usetikzlibrary{fadings}

%\begin{document}

\begin{tikzpicture}

\tikzfading[name=fade right,
left color=transparent!100,
right color=transparent!0]

\tikzfading[name=fade bottom,
top color=transparent!100,
bottom color=transparent!0]


% Inner figure
% Vertical movement
\foreach \y in {1, 3} {
    % Horizontal movement
    \foreach \x in {2, 7} {
        % Components of C_0
        \draw[ultra thin, fill=black!10] (\x,\y) rectangle (\x+2.5,\y+2);
        \draw[ultra thin, fill=black!10] (\x+2.5,\y) rectangle (\x+5,\y+2);

        % Components of C_1
        \fill[color=black!60] (\x+0.5,\y+0.5) rectangle (\x+2,\y+2);
        \fill[color=black!60] (\x+3,\y) rectangle (\x+4.5,\y+1.5);

        % Level sets
        \foreach \z in {0.25, 0.5, ..., 1} {
            \draw[color=black!30] (\x,\y+\z) -- (\x+0.5,\y+\z*0.5) -- (\x+2,\y+\z*0.5) -- (\x+2.5,\y+\z) -- (\x+3,\y+\z*1.5) -- (\x+4.5,\y+\z*1.5) -- (\x+5,\y+\z);
            \draw[color=black!30] (\x,\y+2-\z) -- (\x+0.5,\y+2-\z*1.5) -- (\x+2,\y+2-\z*1.5) -- (\x+2.5,\y+2-\z) -- (\x+3,\y+2-\z*0.5) -- (\x+4.5,\y+2-\z*0.5) -- (\x+5,\y+2-\z);
        }
        
    }
}

% Small dashes outside the figure
\foreach \y in {1, 1.25, ..., 5} {
    \draw[color=black!30] (1.75,\y) -- (2,\y);
}

% y_0 and other highlited level sets
\foreach \y in {3} {
\draw[thick] (2-0.25,\y+1.5) -- (2,\y + 1.5);
\foreach \x in {2,7} {
\foreach \z in {0, 0.5, 1} {
\draw[thick] (\x,\y+2-\z) -- (\x+0.5,\y+2-\z*1.5) -- (\x+2,\y+2-\z*1.5) -- (\x+2.5,\y+2-\z) -- (\x+3,\y+2-\z*0.5) -- (\x+4.5,\y+2-\z*0.5) -- (\x+5,\y+2-\z);
}
}
}

% Subscription
\node[font=\large,anchor=east] at (1.75,4.5) {$y_0$};
\draw (2,5) -- (0.9,5);
\draw[<->] (1,5) -- node[midway,font=\Large, anchor=east]{$I^{(n)}$} (1,4);
\draw (2,4) -- (0.9,4);

% Fade
\fill[white,path fading=fade bottom] (1.5,1.49) rectangle (10.5,4);
\fill[white] (1.5,0.9) rectangle (10.5,1.5);
\fill[white,path fading=fade right] (7,0.9) rectangle (10.5,5.1);
\fill[white] (10.4,0.9) rectangle (12.1,5.1);

% Subscriptions



\end{tikzpicture}

%\end{document}
